NLLG Quarterly arXiv Report 06/23: What are the most influential current AI Papers?

The rapid growth of information in the field of Generative Artificial Intelligence (AI), particularly in the subfields of Natural Language Processing (NLP) and Machine Learning (ML), presents a significant challenge for researchers and practitioners to keep pace with the latest developments. To address the problem of information overload, this report by the Natural Language Learning Group at Bielefeld University focuses on identifying the most popular papers on arXiv, with a specific emphasis on NLP and ML. The objective is to offer a quick guide to the most relevant and widely discussed research, aiding both newcomers and established researchers in staying abreast of current trends. In particular, we compile a list of the 40 most popular papers based on normalized citation counts from the first half of 2023. We observe the dominance of papers related to Large Language Models (LLMs) and specifically ChatGPT during the first half of 2023, with the latter showing signs of declining popularity more recently, however. Further, NLP related papers are the most influential (around 60\% of top papers) even though there are twice as many ML related papers in our data. Core issues investigated in the most heavily cited papers are: LLM efficiency, evaluation techniques, ethical considerations, embodied agents, and problem-solving with LLMs. Additionally, we examine the characteristics of top papers in comparison to others outside the top-40 list (noticing the top paper's focus on LLM related issues and higher number of co-authors) and analyze the citation distributions in our dataset, among others.

==> structure/0201_someotherstuff.tex <==
\subsection*{Analysis} 




\iffalse
\begin{figure}[H] % Exemplo de imagem
					\vspace*{-1cm}
					\includegraphics[width=\linewidth]{regression.png}
\end{figure}
\vspace{0.5cm}
\fi 




\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/mean_citation_counts_by_week_all (3).png}
    \caption{Weekly Mean Citation for papers in the last 7 months}
    \label{fig:}
\end{figure}



%Surprisingly, the LG category appears to be underrepresented in terms of citation counts.
%On the other hand, the CL category exhibits higher citation counts on average, particularly at the beginning of the year, indicating a strong presence and popularity of papers in this domain. Although some papers were categorized under both AI and LG, we focused primarily on their primary category to ensure a more focused representation.
%\todo{SE: check this}
%\vspace{1cm}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/mean_count_categories_count.png}
    \caption{Weekly overview of number of papers published in the last 7 months by category}
    \label{fig:}
\end{figure}



%\vspace{1cm}






Based on the figures and analysis, it is evident that the terms "ChatGPT" and "LLMs" show a more pronounced presence in the titles and abstracts of papers within the cs.AI category compared to cs.LG. However, both cs.AI and cs.LG categories exhibit a lower rate of appearance of these terms when compared to the cs.CL category.

The cs.CL category demonstrates a notable increase and subsequent decrease in the occurrence of the terms over time, indicating a stronger correlation with the publication of papers and mean citation counts compared to the other categories.

On the other hand, while cs.AI shows a relatively higher presence of the terms, it does  follow the same significant pattern of increase and decrease as in cs.CL. Similarly, cs.LG shows even lower rates of appearance of the terms and lacks a clear pattern of increase and decrease over time.

These observations suggest that cs.AI has a relatively higher association with the terms "ChatGPT" and "LLMs" compared to cs.LG, but both categories exhibit lower rates of term occurrence when compared to cs.CL. Further investigation is needed to understand the underlying reasons behind these differences and their potential impact on the publication dynamics and citation means within each specific category.

\begin{figure}[h] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=0.5\linewidth]{structure/pics/terms_chatgpt (1).pdf}
    \includegraphics[width=0.5\linewidth]{structure/pics/terms_llm (1).pdf}
    \includegraphics[width=0.5\linewidth]{structure/pics/terms_llama (1).pdf}
    \includegraphics[width=0.5\linewidth]{structure/pics/terms_only_categories_chatGPT.pdf}
    \caption{Terms in title and abstract for all papers. Top left: ``GPT'', top right: ``LLMs''. Bottom left: ``LLAMA''. Bottom right: ``ChatGPT''.}
    \label{fig:}
\end{figure}
%\vspace{1cm}

%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/terms_llm (1).pdf}
%    \caption{Terms LLMs in title and abstract for all papers}
%    \label{fig:}
%\end{figure}

%\vspace{1cm}

%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/terms_llama (1).pdf}
%    \caption{Terms LLAMA in title and summary for all papers}
%    \label{fig:}
%\end{figure}
%plot terms by category
%\vspace{1cm}
%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/terms_only_categories_chatGPT.pdf}
%    \caption{Terms chatGPT in title and summary for papers  filtered  by the 3  categories}
%    \label{fig:}
%\end{figure}
%\vspace{1cm}
%
%\begin{figure}[h] % Exemplo de imagem
%	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics%/terms_only_categories_llm.pdf}
%    \caption{Terms LLM in title and summary for papers filtered  by the 3  categories}
%    \label{fig:}
%\end{figure}

%\vspace{1cm}
\begin{figure}[h] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/terms_only_categories_llama (1).pdf}
    \caption{Terms LLAMA in title and summary for papers  filtered  by the 3  categories}
    \label{fig:}
\end{figure}

Based on the figures and analysis, we can observe a clear pattern in the occurrence of the terms "ChatGPT" and "LLMs" within the titles and abstracts of the papers. In the case of category cs.CL, there is a notable increase and subsequent decrease in the appearance of these terms over time, alongside a corresponding trend in the publication of papers and mean citation counts. This indicates a potential relationship between the terms' prevalence, paper publication, and citation counts within the cs.CL category. The other categories, cs.LG and cs.AI, also show distinctive patterns, suggesting different trends in term usage, paper publication, and citation means within each specific category.


\vspace{1cm}


\begin{figure}[h] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/terms_by_category (1).png}
    \caption{Terms gpt or LLMs in title and summary by category}
    \label{fig:}
\end{figure}




%\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
%	\includegraphics[width=\linewidth]{structure/pics/papers_published_by_timeWeek_all.png}
 %   \caption{Weekly overview of number of papers published in the last 7 months}
  %  \label{fig:}
%\end{figure}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/papers_published_by_time_all_Month.pdf}
    \caption{Overall number of papers published in the last 7 months}
    \label{fig:}
\end{figure}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/mean_count_categories_sorted_month.pdf}
    \caption{Overall number of papers published in the last 7 months}
    \label{fig:}
\end{figure}

\begin{figure}[htb] % Exemplo de imagem
	%\vspace*{-1cm}
	\includegraphics[width=\linewidth]{structure/pics/papers_over_time_until_july.pdf}
    \caption{Number of Papers published in the last 7 months by different categories}
    \label{fig:}
\end{figure}

==> structure/04_analysis.tex <==
\section{Analysis of top list}

Upon analyzing the top 20 papers in the fields of Artificial Intelligence (AI), Computational Linguistics (CL), and Machine Learning (LG), a notable trend emerges with regard to citation counts. It is evident that CL papers tend to have higher citation counts compared to their counterparts in AI and LG.

One plausible explanation for this observation is the surge in popularity and attention surrounding topics like ChatGPT, ChatGPT3-4, and large language models in recent times. ChatGPT, in particular, has garnered widespread interest from researchers, practitioners, and the general public due to its impressive language generation capabilities and versatile applications.

As a result, many research efforts have been dedicated to advancing language models in the context of computational linguistics, leading to a substantial increase in citations for relevant papers. Additionally, the prolific development of AI language models and their potential impact on various domains has sparked widespread interest and contributed to the higher citation counts in CL.

It is noteworthy that some papers, like the "PaLM 2 Technical Report," are categorized under both AI and CL, reflecting the interdisciplinary nature of research in the domain of large language models. Despite belonging to multiple categories, the primary classification of such papers under CL underscores the emphasis on language processing and understanding.
\vspace{3cm}

\begin{figure}[h!] % Exemplo de imagem
					\vspace*{-1cm}
					\includegraphics[width=\linewidth]{mean_citation_bycategories_box.png}
\end{figure}



The diversity of language models in the top 20 papers, including LLaMA, PaLM-2, and GPT-4, showcases the rich landscape of LLMs and the variety of approaches employed by researchers to tackle complex language processing tasks. Each model brings its unique strengths and contributions to the table, providing a broad range of tools and techniques for researchers to explore and leverage.

Based on the top papers, we can observe that the research in the field of language models can be classified into various categories. These categories include:

1.Technical Reports and Surveys: Several papers are technical reports or surveys, which indicate a focus on presenting research findings, methodologies, or comprehensive overviews of specific topics.
This first Category include  the papers: 
\vspace{0.5cm}
   \begin{itemize}
       \item  PaLM 2 Technical Report
       \item  GPT-4 Technical Report
       \item A Survey of Large Language Models
   \end{itemize}
   

2.Advancements in Language Models: Papers like "LLaMA: Open and Efficient Foundation Language Models," Sparks of Artificial General Intelligence: Early experiments with GPT-4" and "A Watermark for Large Language Models" and "Toolformer: Language Models Can Teach Themselves to Use Tools" suggest a focus on improvements and advancements in language models.


3.Specific Applications in Various Domains: Some of the  papers, such as 
"QLoRA: Efficient Finetuning of Quantized LLMs,"Judging LLM-as-a-judge with MT-Bench and Chatbot Arena" and  "Mathematical Capabilities of ChatGPT"
are focused on specific application areas of language models, such as Named Entity Recognition and Instruction Tuning.

4.Evaluation and Detection of Machine-Generated Text: Papers like "DetectGPT: Zero-Shot Machine-Generated Text Detection using Probability Curvature" and "How Close is ChatGPT to Human Experts? Comparison Corpus, Evaluation, and Detection" indicate a focus on evaluating and detecting machine-generated text. These studies delve into methods and techniques to discern machine-generated content from human-generated content, addressing the vital challenge of detecting the origin of language model outputs. Moreover, this category also explores the fascinating question of how closely language models, such as ChatGPT, resemble human experts in various tasks. Understanding the proximity of these models to human performance can provide valuable insights into their capabilities and limitations, fostering discussions around the boundaries of machine intelligence and human cognition.

5.Ethical and Fairness Concerns: Papers such as "Large Language Models are not Fair Evaluators" suggest a focus on ethical concerns and fairness related to language models. This Paper can be belong as well into category 4 (Evaluation and Detection of Machine-Generated Text)

6.Experimentation and Problem Solving: Titles like "Sparks of Artificial General Intelligence: Early experiments with GPT-4" ,"Tree of Thoughts: Deliberate Problem Solving with Large Language Models" and "Instruction Tuning with GPT-4T" indicate a focus on experimentation and problem-solving using language models. These papers explore the potential of language models, such as GPT-4, in tackling complex problem-solving tasks and shedding light on the emergence of artificial general intelligence. Moreover, specific topics like "Mathematical Capabilities of ChatGPT" delve into the capabilities of GPT models in solving mathematical problems, distinguishing multiple dimensions of mathematical reasoning. This category reflects the exciting frontier of how language models can be leveraged to address various challenges and demonstrate their problem-solving prowess in a range of domains.

7. Exploration of Language Model Potential and Limitations: 
In the realm of implementing ChatGPT in various domains, let's explore some noteworthy papers that shed light on its mathematical capabilities, its potential role as a generic AI task solver and tool usage.
Papers falling, like "Augmented Langauge Models: a Survey", fall under this category, focusing on the reasoning skills and the ability to use tools of LMs.Similarly we have "A Multitask, Multilingual, Multimodal Evaluation of ChatGPT on Reasoning, Hallucination, and Interactivity", present a technical evaluation of ChatGPT.This paper highlights that ChatGPT, like other large language models (LLMs), exhibits strengths and weaknesses in reasoning abilities. Overall, this study sheds light on ChatGPT's reasoning capabilities and brings attention to its tendency for hallucination, providing valuable insights into the model's performance and areas of improvement.

8. Multitasking and Multilingual Capabilities:
This category focuses on the multilingual capabilities of Large Language Models (LLMs). Papers like "SemEval-2023 Task 2: Fine-grained Multilingual Named Entity Recognition (MultiCoNER 2)" explore the identification of complex named entities across 12 languages in different scenarios, including noisy settings. Another paper, "StarCoder: may the source be with you!", evaluates Code LLMs' capabilities comprehensively, demonstrating that StarCoderBase outperforms other open Code LLMs that support multiple programming languages, including the OpenAI code-cushman-001 model.

9. GPT Gaming Interaction":  This category includes papers focusing on the interaction between Large Language Models (LLMs) and gaming environments. One example is the paper "Voyager: An Open-Ended Embodied Agent with Large Language Models," which highlights the skills of Voyager, such as temporally extended, interpretable, and compositional abilities. Voyager's skills compound rapidly and alleviate catastrophic forgetting, leading to strong in-context lifelong learning capability. Notably, Voyager exhibits exceptional proficiency in playing Minecraft, achieving 3.3x more unique accomplishments.


In summary, the top papers demonstrate a clear category clustering for specific domains, highlighting the diverse applications and capabilities of ChatGPT. Papers in the realm of gaming and large language models showcase the integration of LLMs into embodied agents and reinforcement learning algorithms, pushing the boundaries of AI in gaming and other domains.

While some papers offer positive insights into the transformative potential of large language models, others present critical perspectives and highlight existing problems with current models. These contributions collectively showcase the remarkable progress achieved in LLMs, with standout models like LLaMA, PaLM-2, and GPT-4 captivating the research community.

Overall, this analysis reveals the wide range of topics covered by the top selected papers, from foundational language models to advanced applications in specific domains. The significant contributions made by each paper showcase the continuous progress in AI and LLMs, highlighting their potential to reshape the landscape of natural language processing and benefit society at large.











==> structure/abstract_old.tex <==
\begin{abstract}
    The rapid growth of information in the field of Generative Artificial Intelligence (AI), particularly in the subfields of Natural Language Processing (NLP) and Machine Learning (ML), presents a significant challenge for researchers and practitioners to keep pace with the latest developments. To address the problem of information overload, this report by the Natural Language Learning Group at Bielefeld University focuses on identifying the most popular papers on arXiv, with a specific emphasis on NLP and ML. The objective is to offer a quick guide to the most relevant and widely discussed research, aiding both newcomers and established researchers in staying abreast of current trends.
%
%The report leverages the comprehensive and expeditious publication process of arXiv, a prominent pre-print repository, to 
In particular, we compile a list of the 40 most popular papers based on normalized citation counts from the first half of 2023. %Among our key findings, NLP emerges as more influential than ML in terms of citations, despite the presence of more ML papers in the dataset. Notably, 
We observe the dominance of papers related to Large Language Models (LLMs) and specifically ChatGPT during the first half of 2023, with the latter showing signs of declining popularity more recently, however. Further, NLP related papers are the most influential (around 60\% of top papers) even though there are twice as many ML related papers in our data. Core issues investigated in the most heavily cited papers are:  
%
%The investigation delves into various aspects, including 
LLM efficiency, evaluation techniques, ethical considerations, embodied agents, and problem-solving with LLMs. %indicating the focal points of current research interest. 
Additionally, we examine the characteristics of top papers in comparison to others outside the top-40 list (noticing the top paper's focus on LLM related issues and higher number of co-authors) and analyze the citation distributions in our dataset, among others. 
%and track the popularity of ChatGPT, a significant contributor to the recent LLM hype.
%
%The report aims to assist both newcomers and established researchers by providing accessible links to pertinent literature. Future plans include regular updates to observe evolving trends over time, deeper analysis of the arXiv dataset, and the inclusion of other AI-related arXiv categories (e.g., cs.CV, stat.ML, cs.AI). The open availability of code and data from this study contributes to the advancement of the field and fosters collaboration among researchers in the AI community.
\end{abstract}


==> structure/tables/top20_se.tex <==
 \begin{table}[htb]
 \centering
 \small 
 \begin{tabular}{|p{0.3cm}|p{5.5cm}|p{1cm}|p{4.5cm}|p{0.7cm}|p{0.5cm}|p{1cm}|}
\toprule
 No. & Title & Cat. & Link & Week & Cit&  zscore \\ \midrule
%1 & LLaMA: Open and Efficient Foundation Language Models & cs.CL & 
%\url{http://arxiv.org/abs/2302.13971v1} & 9 & 852 & 28.016 \\
%2 & PaLM 2 Technical Report & cs.CL & \url{http://arxiv.org/abs/2305.10403v1} 
1 & LLaMA: Open and Efficient Foundation Language Models & cs.CL & \url{http://arxiv.org/abs/2302.13971v1} & 9 & 852 & 28.016\\
2 & PaLM 2 Technical Report & cs.CL & \url{http://arxiv.org/abs/2305.10403v1} & 20 & 82 & 25.479\\
3 & GPT-4 Technical Report & cs.CL & \url{http://arxiv.org/abs/2303.08774v3} & 11 & 507 & 25.365\\
4 & Sparks of Artificial General Intelligence: Early experiments with GPT-4 & cs.CL & \url{http://arxiv.org/abs/2303.12712v5} & 12 & 348 & 24.332\\
5 & PaLM-E: An Embodied Multimodal Language Model & cs.LG & \url{http://arxiv.org/abs/2303.03378v1} & 10 & 162 & 21.135\\
6 & QLoRA: Efficient Finetuning of Quantized LLMs & cs.LG & \url{http://arxiv.org/abs/2305.14314v1} & 21 & 30 & 20.411\\
7 & Segment Anything & cs.CV & \url{http://arxiv.org/abs/2304.02643v1} & 14 & 162 & 18.425\\
8 & A Multitask, Multilingual, Multimodal Evaluation of ChatGPT on Reasoning, Hallucination, and Interactivity & cs.CL & \url{http://arxiv.org/abs/2302.04023v2} & 6 & 212 & 16.831\\
9 & A Survey of Large Language Models & cs.CL & \url{http://arxiv.org/abs/2303.18223v11} & 13 & 166 & 16.504\\
10 & Judging LLM-as-a-judge with MT-Bench and Chatbot Arena & cs.CL & \url{http://arxiv.org/abs/2306.05685v2} & 23 & 18 & 16.173\\
11 & Visual Instruction Tuning & cs.CV & \url{http://arxiv.org/abs/2304.08485v1} & 16 & 89 & 15.341\\
12 & Tree of Thoughts: Deliberate Problem Solving with Large Language Models & cs.CL & \url{http://arxiv.org/abs/2305.10601v1} & 20 & 47 & 14.519\\
13 & Toolformer: Language Models Can Teach Themselves to Use Tools & cs.CL & \url{http://arxiv.org/abs/2302.04761v1} & 6 & 174 & 13.776\\
14 & How Close is ChatGPT to Human Experts? Comparison Corpus, Evaluation, and Detection & cs.CL & \url{http://arxiv.org/abs/2301.07597v1} & 3 & 93 & 13.716\\
15 & Extracting Training Data from Diffusion Models & cs.CR & \url{http://arxiv.org/abs/2301.13188v1} & 5 & 97 & 13.639\\
16 & Voyager: An Open-Ended Embodied Agent with Large Language Models & cs.AI & \url{http://arxiv.org/abs/2305.16291v1} & 21 & 20 & 13.495\\
17 & Large Language Models are not Fair Evaluators & cs.CL & \url{http://arxiv.org/abs/2305.17926v1} & 22 & 13 & 12.911\\
18 & HuggingGPT: Solving AI Tasks with ChatGPT and its Friends in Hugging Face & cs.CL & \url{http://arxiv.org/abs/2303.17580v3} & 13 & 129 & 12.777\\
19 & A Watermark for Large Language Models & cs.LG & \url{http://arxiv.org/abs/2301.10226v3} & 4 & 76 & 12.606\\
20 & DetectGPT: Zero-Shot Machine-Generated Text Detection using Probability Curvature & cs.CL & \url{http://arxiv.org/abs/2301.11305v2} & 4 & 75 & 12.436\\
\bottomrule
 \end{tabular}
 \caption{Papers, their prime category, arXiv link, week of first arXiv submission, citation count (as of 07/27/2023) and zscore. \textbf{Top 20 papers} according to zscore among all cs.CL, cs.AI and cs.LG papers.}
 \label{table:top20}
 \end{table}

==> structure/tables/top40_se.tex <==

\begin{table}[htb]
 \centering
 \footnotesize
 \begin{tabular}{|p{0.3cm}|p{5.5cm}|p{1cm}|p{4.5cm}|p{0.7cm}|p{0.5cm}|p{1cm}|}
\toprule
 No. & Title & Cat. & Link & Week & Cit&  zscore \\ \midrule
21 & Mastering Diverse Domains through World Models & cs.AI & \url{http://arxiv.org/abs/2301.04104v1} & 2 & 59 & 12.340\\
22 & A Comprehensive Survey on Pretrained Foundation Models: A History from BERT to ChatGPT & cs.AI & \url{http://arxiv.org/abs/2302.09419v3} & 7 & 79 & 12.134\\
23 & Augmented Language Models: a Survey & cs.CL & \url{http://arxiv.org/abs/2302.07842v1} & 7 & 79 & 12.134\\
24 & ImageBind: One Embedding Space To Bind Them All & cs.CV & \url{http://arxiv.org/abs/2305.05665v2} & 19 & 38 & 11.765\\
25 & T2I-Adapter: Learning Adapters to Dig out More Controllable Ability for Text-to-Image Diffusion Models & cs.CV & \url{http://arxiv.org/abs/2302.08453v2} & 7 & 76 & 11.662\\
26 & Is ChatGPT a General-Purpose Natural Language Processing Task Solver? & cs.CL & \url{http://arxiv.org/abs/2302.06476v2} & 6 & 144 & 11.365\\
27 & SemEval-2023 Task 2: Fine-grained Multilingual Named Entity Recognition (MultiCoNER 2) & cs.CL & \url{http://arxiv.org/abs/2305.06586v2} & 19 & 36 & 11.131\\
28 & Mathematical Capabilities of ChatGPT & cs.LG & \url{http://arxiv.org/abs/2301.13867v2} & 5 & 79 & 11.051\\
29 & The Flan Collection: Designing Data and Methods for Effective Instruction Tuning & cs.AI & \url{http://arxiv.org/abs/2301.13688v2} & 5 & 78 & 10.907\\
30 & Video-LLaMA: An Instruction-tuned Audio-Visual Language Model for Video Understanding & cs.CL & \url{http://arxiv.org/abs/2306.02858v3} & 23 & 12 & 10.702\\
31 & InstructBLIP: Towards General-purpose Vision-Language Models with Instruction Tuning & cs.CV & \url{http://arxiv.org/abs/2305.06500v2} & 19 & 33 & 10.181\\
32 & The RefinedWeb Dataset for Falcon LLM: Outperforming Curated Corpora with Web Data, and Web Data Only & cs.CL & \url{http://arxiv.org/abs/2306.01116v1} & 22 & 10 & 9.855\\
33 & Distilling Step-by-Step! Outperforming Larger Language Models with Less Training Data and Smaller Model Sizes & cs.CL & \url{http://arxiv.org/abs/2305.02301v2} & 18 & 24 & 9.776\\
34 & mPLUG-Owl: Modularization Empowers Large Language Models with Multimodality & cs.CL & \url{http://arxiv.org/abs/2304.14178v1} & 17 & 34 & 9.506\\
35 & Theory of Mind May Have Spontaneously Emerged in Large Language Models & cs.CL & \url{http://arxiv.org/abs/2302.02083v3} & 5 & 68 & 9.470\\
36 & Otter: A Multi-Modal Model with In-Context Instruction Tuning & cs.CV & \url{http://arxiv.org/abs/2305.03726v1} & 18 & 23 & 9.353\\
37 & SemEval-2023 Task 7: Multi-Evidence Natural Language Inference for Clinical Trial Data & cs.CL & \url{http://arxiv.org/abs/2305.02993v2} & 18 & 23 & 9.353\\
38 & The False Promise of Imitating Proprietary LLMs & cs.CL & \url{http://arxiv.org/abs/2305.15717v1} & 21 & 14 & 9.346\\
39 & PandaGPT: One Model To Instruction-Follow Them All & cs.CL & \url{http://arxiv.org/abs/2305.16355v1} & 21 & 14 & 9.346\\
40 & ChatGPT is not all you need. A State of the Art Review of large Generative AI models & cs.LG & \url{http://arxiv.org/abs/2301.04655v1} & 2 & 45 & 9.323\\
\bottomrule
 \end{tabular}
 \caption{Papers, their prime category, arXiv link, week of first arXiv submission, citation count (as of 07/27/2023) and zscore. \textbf{Papers 21-40} according to zscore among all cs.CL, cs.AI and cs.LG papers.}
 \label{table:top40}
 \end{table}

==> structure/tables/toppapers_vf.tex <==
\begin{tabular}
{|p{0.3cm}|p{5.5cm}|p{1cm}|p{5.5cm}|p{0.5cm}|p{0.5cm}|p{1cm}|}
\toprule

 No. & title & category &paper& week & cnt&  Nmean \\
\midrule
   1 &                            PaLM 2 Technical Report &            cs.CL &  http://arxiv.org/abs/2305.10403v1 &    20 &               82 &           22.14 \\
   2 & LLaMA: Open and Efficient Foundation Language M... &            cs.CL &  http://arxiv.org/abs/2302.13971v1 &     9 &              852 &           22.11 \\
   3 &                             GPT-4 Technical Report &            cs.CL &  http://arxiv.org/abs/2303.08774v3 &    11 &              507 &           19.77 \\
   4 &      QLoRA: Efficient Finetuning of Quantized LLMs &            cs.LG &  http://arxiv.org/abs/2305.14314v1 &    21 &               30 &           18.82 \\
   5 & Sparks of Artificial General Intelligence: Earl... &            cs.CL &  http://arxiv.org/abs/2303.12712v5 &    12 &              348 &           18.72 \\
   6 &      PaLM-E: An Embodied Multimodal Language Model &            cs.LG &  http://arxiv.org/abs/2303.03378v1 &    10 &              162 &           16.43 \\
   7 & Judging LLM-as-a-judge with MT-Bench and Chatbo... &            cs.CL &  http://arxiv.org/abs/2306.05685v2 &    23 &               18 &           15.96 \\
   8 & SemEval-2023 Task 2: Fine-grained Multilingual ... &            cs.CL &  http://arxiv.org/abs/2305.06586v2 &    19 &               36 &           15.01 \\
   9 & A Multitask, Multilingual, Multimodal Evaluatio... &            cs.CL &  http://arxiv.org/abs/2302.04023v2 &     6 &              212 &           14.78 \\
  10 &                  A Survey of Large Language Models &            cs.CL & http://arxiv.org/abs/2303.18223v11 &    13 &              166 &           13.04 \\
  11 &              A Watermark for Large Language Models &            cs.LG &  http://arxiv.org/abs/2301.10226v3 &     4 &               76 &           12.64 \\
  12 & Tree of Thoughts: Deliberate Problem Solving wi... &            cs.CL &  http://arxiv.org/abs/2305.10601v1 &    20 &               47 &           12.60 \\
  13 & DetectGPT: Zero-Shot Machine-Generated Text Det... &            cs.CL &  http://arxiv.org/abs/2301.11305v2 &     4 &               75 &           12.47 \\
  14 & Voyager: An Open-Ended Embodied Agent with Larg... &            cs.AI &  http://arxiv.org/abs/2305.16291v1 &    21 &               20 &           12.43 \\
  15 &      Large Language Models are not Fair Evaluators &            cs.CL &  http://arxiv.org/abs/2305.17926v1 &    22 &               13 &           12.29 \\
  16 & Toolformer: Language Models Can Teach Themselve... &            cs.CL &  http://arxiv.org/abs/2302.04761v1 &     6 &              174 &           12.10 \\
  17 &                      Instruction Tuning with GPT-4 &            cs.CL &  http://arxiv.org/abs/2304.03277v1 &    14 &               81 &           11.84 \\
  18 & How Close is ChatGPT to Human Experts? Comparis... &            cs.CL &  http://arxiv.org/abs/2301.07597v1 &     3 &               93 &           11.62 \\
  19 &             StarCoder: may the source be with you! &            cs.CL &  http://arxiv.org/abs/2305.06161v1 &    19 &               28 &           11.61 \\
  20 &               Mathematical Capabilities of ChatGPT &            cs.LG &  http://arxiv.org/abs/2301.13867v2 &     5 &               79 &           11.22 \\
\bottomrule

\end{tabular}
 

 


 










